On the Hybrid Extension of CTL and CTL+

The paper studies the expressivity, relative succinctness and complexity of satisfiability for hybrid extensions of the branching-time logics CTL and CTL+ by variables. Previous complexity results show that only fragments with one variable do have elementary complexity. It is shown that H1CTL+ and H1CTL, the hybrid extensions with one variable of CTL+ and CTL, respectively, are expressively equivalent but H1CTL+ is exponentially more succinct than H1CTL. On the other hand, HCTL+, the hybrid extension of CTL with arbitrarily many variables does not capture CTL*, as it even cannot express the simple CTL* property EGFp. The satisfiability problem for H1CTL+ is complete for triply exponential time, this remains true for quite weak fragments and quite strong extensions of the logic.

==> compl-hctl+-old-version.tex <==
----begin-old-version--------------
\newline
\textit{Formulation of a winning strategy for player E}
\newline
The formula $\varphi_I$ is composed of the conjunction of $\chi$ and $\psi$ where 
%$\chi = \bigwedge_{i=1}^{10} \chi_i$ 
the first one describes the basic tree structure that is needed to formulate a strategy and 
%$\psi=\bigwedge_{i=1}^{10} \psi_i$
the second one guarantees that the model of $\varphi_I$ corresponds to a winning strategy for player E. Beside a textual description of the properties needed to be expressed we give the logical formulation only in cases which are not obvious.
W start with the components of $\chi$. The first property helps to formulate further properties in a facile way.     
\newcommand{\ourcondition}[2]{#1: \emph{#2}}
%In order to make some properties easy to formulate in the sequel, we first state that each node of the tree is labelled with %exactly one of the propositions $q_{row}$, $q_{pos}$, $q_{\sharp}$, $o$ and $c$.      
\newline
\newline
\ourcondition{T1}{Each node of the tree is labelled with exactly one of the propositions $q_{row}$, $q_{pos}$, $q_{\sharp}$, $o$ and $c$.}
%\begin{align*}
%\chi_1 = AG [&(q_{row} \vee q_{pos} \vee q_{\sharp} \vee o \vee c) \wedge \\ 
%&(q_{row} \rightarrow \neg q_{pos} \wedge \neg q_{\sharp} \wedge \neg o \wedge \neg c) \wedge  \\
%&(q_{pos} \rightarrow \neg q_{row} \wedge \neg q_{\sharp} \wedge \neg o \wedge \neg c) \wedge \\
%&(q_{\sharp} \rightarrow \neg q_{row} \wedge \neg q_{pos} \wedge \neg o \wedge \neg c) \wedge \\
%&(o \rightarrow \neg q_{row} \wedge \neg q_{pos} \wedge \neg q_{\sharp} \wedge \neg c) \wedge \\         
%&(c \rightarrow \neg q_{row} \wedge \neg q_{pos} \wedge \neg q_{\sharp} \wedge \neg o)]  
%\end{align*}
\newline
\newline
\ourcondition{T2}{The root induces with the proposition $q_{row}$ the encoding of the first row and every node labelled with $q_{row}$ has exactly one child labled with $q_{pos}$ signalising the encoding of a new position.}   
\begin{align*}  
\chi_2 =& q_{row} \wedge AG[q_{row} \rightarrow EX (q_{pos} \wedge \dx.@_{\myroot} EF(EX x \wedge AX x))]
\end{align*}
\ourcondition{T3}{Every child of a $q_{pos}$-node is labelled with the initial digit number.}
%\ourcondition{T3}{Every child of a $q_{pos}$-node starts the inner counter.}
\begin{align*}  
\chi_3 = AG[q_{pos} \rightarrow AX(o \wedge \bigwedge_{i=0}^{n-1} \neg b_i)]
\end{align*}
\ourcondition{T4}{As long as the last bit node of a position is not reached, the next node is labelled with the next digit number.}
%\ourcondition{T4}{As long as the last bit node of a position is not reached, the inner counter is increased by one bit.} 
\begin{align*} 
\chi_4 = AG&[o \wedge \neg \bigwedge _{i=0}^{n-1} b_i \rightarrow \\
&             \dx.EX(o \wedge \bigvee_{i=0}^{n-1} 
(\bigwedge _{j<i} (\neg b_j \wedge @_x b_j)\wedge b_i \wedge @_x \neg b_i \wedge \bigwedge _{j>i} (b_j \leftrightarrow @_x b_j)))]
\end{align*}
\ourcondition{T5}{Each position bit has a child, which represents a copy of it. The nodes of a subtree rooted at a copy node are labelled exactly with the same propositions.}
\begin{align*} 
\chi_5 = AG[&(o \rightarrow \dx. EX (c \wedge \bigwedge_{i=0}^{n-1}(b_i \leftrightarrow @_x b_i) \wedge b \leftrightarrow @_x b)) \wedge \\
&(c \rightarrow \dx.AG (c \wedge \bigwedge_{i=0}^{n-1}(b_i \leftrightarrow @_x b_i) \wedge b \leftrightarrow @_x b))]
\end{align*}
\ourcondition{T6}{Each position bit has exactly two childs. One of them is its copy node and the other one is:  
\begin{itemize}
\item the next position bit if the current node is not already the last position bit or
\item a node containing one of the propositions $q_{pos}$, $q_{row}$ and $q_{\sharp}$, otherwise.
\end{itemize}}
%The next two formulas express that each position bit has in addition to its unique copy node exactly one further child node:
%\begin{itemize}
%\item The next position bit if the current node is not already the last position bit ($\chi_3$), or
%\item a node containing one of the propositions $q_{pos}$, $q_{row}$ and $q_{\sharp}$ ($\chi_4$).
%\end{itemize} 
%Whether the last position bit is reached, depends on the value of the inner counter. Whether a new position or a new row ist started, depends on the value of the outer counter. These counters will be defined below.
%
%\ahmet{Perhaps we should already say here that the outer counter not necessarily has to ,,count'': In the case that player A cannot make a move.}
%
%In order to say that \emph{exactly one} node with a certain property exists, we have to use the $\dx$-operator.
%\begin{align*} 
%\chi_3 = AG[o \wedge \neg \bigwedge_{i=0}^{n-1} b_i \rightarrow  &EX(o \wedge \downarrow x. @_{root} EF(EXx \wedge AX(o \rightarrow x))) \wedge \\
%                                                                 	    &EX(c \wedge \downarrow x. @_{root} EF(EXx \wedge AX(c \rightarrow x))) \wedge  \\
%																																	    &AX(o \vee c)]  \\
%\chi_4 = AG[o \wedge \bigwedge_{i=0}^{n-1} b_i \rightarrow &EX(c \wedge \downarrow x. @_{root}EF(EXx \wedge AX(c \rightarrow x))) \wedge \\
%																															&[EX(q_{pos} \wedge \downarrow x. @_{root} EF(EXx \wedge AX(q_{pos} \rightarrow x))) \wedge \\ & \neg EX q_{row} \wedge \neg EX q_{\sharp} \vee  \\
%																															& EX(q_{row} \wedge \downarrow x. @_{root} EF(EXx \wedge AX(q_{row} \rightarrow x))) \wedge \\ & \neg EX q_{\sharp} \wedge \neg EX q_{pos} \vee  \\
%																															& EX(q_{\sharp} \wedge \downarrow x. @_{root} EF(EXx \wedge AX(q_{\sharp} \rightarrow x))) \wedge \\ & \neg EX q_{pos} \wedge \neg EX q_{row}  ] \wedge \\
%																															& AX(c \vee q_{row} \vee q_{pos} \vee q_{\sharp})]
%\end{align*}
\ourcondition{T7}{With the proposition $q_{row}$ the counting of the positions of the current row starts. This means that the next position gets the initial position number. Therefore the proposition $b$ is set to false in every bit node of this position.} 
%\ourcondition{T7}{The proposition $q_{row}$ starts the outer counter. This means that the proposition $b$ is set to false in every bit node of the first position of the induced row.} 
\begin{align*}
\chi_7 = AG[q_{row} \rightarrow EX (q_{pos} \wedge AXE((o \wedge \neg b) U (\neg o \wedge \neg c)))]
\end{align*}

Compared to the increasing of a digit number the increasing of a position number is a little bit complicated because in the latter case the bits are distributed over several nodes. In addition, we have to account for the case that player A cannot make a move without violating the horizontal or vertical constraints. In this case the game is over and $q_{\sharp}$-nodes follow only.

We describe the increasing of a position number in three parts.
\newline
\newline
\ourcondition{T8a}{If the last position is reached then a new row is started or the game is over.}     
\begin{align*}
\chi_{8a} = &AG[o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \wedge E((o \wedge b) U (\neg o \wedge \neg c)) \rightarrow E((o \wedge b)U(q_{row} \vee q_{\sharp}))]
\end{align*}
\ourcondition{T8b}{If the last position is not reached and it is the turn of player E then the next position definitely has to be encoded and it gets the next position number.}
\begin{align*}
\chi_{8b} = &AG [o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \wedge  E(oU(o \wedge \neg b)) \wedge \neg E(oU (o \wedge \bigwedge_{i=0}^{n-1}b_i \wedge \neg b)) \rightarrow  \theta]
\end{align*}
\begin{align*}
\theta = &E(oUq_{pos}) \wedge (\mbox{could be eliminated})\\
&      E[oU(o \wedge \neg b \wedge EXE((o\wedge b)Uq_{pos})\wedge \\
&\ \  \ \ \ \ \ \ \dx.[E(oU(q_{pos} \wedge AXE(oU(o \wedge \bigwedge_{i=0}^{n-1}(b_i \leftrightarrow @_x b_i)\wedge b \wedge \\
&\ \  \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \ \ \  \ \ \ \ \ \ \ \ EXE((o \wedge \neg b)U(q_{pos} \vee q_{\sharp} \vee q_{row})))))) \\ 
&\ \ \ \ \ \ \ \ \ \ \ \ \ \wedge @_{root}EF(o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \wedge \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ E[(\dx.E(oU[q_{pos} \wedge AXE (oU (\bigwedge_{i=0}^{n-1}(b_i \leftrightarrow @_x b_i) \wedge b \leftrightarrow @_x b))]))Ux]\ )])]	
\end{align*}
\ourcondition{T8c}{If the last position is not reached and it is the turn of player A then the next position has not necessarily to be encoded but the game could be over.}
\begin{align*}
\chi_{8c} = &AG [o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \wedge E(oU (o \wedge \bigwedge_{i=0}^{n-1}b_i \wedge \neg b)) \rightarrow E(oUq_{\sharp} )\vee \theta] 
\end{align*}

We now use the tree structure described above to encode a winning strategy for player E.
\newline
\newline
\ourcondition{W1}{The game ends after a finite sequence of moves.}
\newline
We express this by postulating that on every rootpath which does not contain any copy nodes a $q_{\sharp}$-node is eventually reached. A $q_{\sharp}$-node is followed only by $q_{\sharp}$-nodes.
\begin{align*} 
\psi_1 = &A(G \neg c \rightarrow F q_{\sharp}) \wedge AG(q_{\sharp} \rightarrow AG q_{\sharp})		
\end{align*}
\ourcondition{W2}{To each position belongs exactly one tile type.}   
\newline
We remember that a tile type $t$ is represented by the proposition $p_t$ in the first bit node of the corresponding position. 
\begin{align*}
\psi_2 = AG[o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \rightarrow \bigvee_{t\in T}(p_t \wedge \bigwedge_{t\neq t' \in T} \neg p_{t'})]
\end{align*}
\ourcondition{W3}{According to the horizontal constraints, the tile type of every position, except the first one on each row, is convenient to the tile type of the precedent position.}
\begin{align*}
\psi_3 = AG(& o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \wedge E(oU(o\wedge b)) \rightarrow \\
&\bigwedge_{t'\in T}[p_{t'} \rightarrow \dx.@_{root} EF(o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \wedge E(oU(q_{pos} \wedge EXx))\wedge \bigvee_{(t,t')\in H} p_t)])
\end{align*}
\ourcondition{W4}{According to the vertical constraints, for every row, except the first one, it holds that the tile type of every position on this row is convenient to the tile type of the same position on the precedent row.}
\newline
The description of the vertical constraints requires the identification of two positions with the same position number on two consecutive rows. This means that two sequences of position bits have to be compared regarding $n+1$ propositions. To be able to do this without causing an exponential blowup in the formula length, we have to fix one of the two sequences as well as one of the two nodes which are currently compared. 
Let $r$ be a sub-path representing a row an $r'$ a sub-path representing the directly preceding row. Let $s$ be the sequence of position bits of a position on $r$ for which the conformance to the vertical constraints has to be guaranteed. To this we first put the variable $x$ to the last node of $s$. To assure that a sequence $s'$ of position bits on $r'$ is adequate to $s$ we require for each node $v'$ in $s'$: there is path that starts in $v'$ and follows the copy nodes of some node $v$ on $s$ so that the propositions in $v'$ and in one of the copy nodes are identical (except for $o$ and $c$). Bacause on such a path the node $v$ can be considered as ''fixed'' and because the description of a path through a boolean combination of temporal operators is allowed in \Honeplus the comparison of $v$ and $v'$ can be performed in the scope of a path quantifier without an exponential blowup in the formula length.
\begin{align*}
\psi_4= & AG(\bigwedge_{t' \in T}(o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \wedge p_{t'} \rightarrow E(oU(o \wedge \bigwedge_{i=0}^{n-1} b_i \wedge \dx.@_{root}AG(\xi \rightarrow  \bigvee_{(t,t') \in V} p_t)))))\\ 
\xi = & o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \wedge E(\neg q_{row} U (q_{row} \wedge EXE (\neg q_{row} U x))) \wedge   \\
  & E[(o \wedge E[G(\neg c \rightarrow Fx) \wedge FE(oUx) \wedge \bigwedge_{i=0}^{n-1}(b_i \leftrightarrow F(c \wedge b_i ))\wedge b \leftrightarrow F(c \wedge b)])U(q_{pos} \vee q_{row})]
\end{align*}
\ahmet{We should say in the definition of the logic what a state formula in the scope of a path quantifier means: The state formula holds in the first node of the path}
\ourcondition{W5}{All possible moves of player A are represented in the encoding.}
%\ourcondition{W5}{A winning strategy for player E has to deliver a countermove for all possible moves of player A.
%The following formula expresses that all possible moves of A are represented.} 
\begin{align*}
\psi_5 = &AG(o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \wedge E(oU(o \wedge \bigwedge_{i=0}^{n-1} b_i \wedge \neg b)) \rightarrow \\
&\ \ \ \ \ \ \bigwedge_{t \in T}(p_t \rightarrow \bigwedge_{(t,t') \in H}(E(oU(q_{pos} \wedge EX p_{t'})) \vee \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ E(oU(o \wedge \bigwedge_{i=0}^{n-1} b_i \wedge \\ 
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \dx. @_{root} EF(\xi \wedge \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \bigvee_{(t'',t')\notin V}(E(oU(q_{pos} \wedge EX(EFx \wedge p_{t''})))))))))) \\
\end{align*}
\ourcondition{W6}{All tile types in the first row are from the set $F$.} 
\begin{align*}
\psi_6 = & AG(  o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \wedge \dx.@_{root} EXE(\neg q_{row} U x ) \rightarrow \bigvee_{t \in F} p_t)
\end{align*} 
\ourcondition{W7}{Unless the game terminates prematurely (because player A is not able to make a further move) all tile types in the last row are from the set $L$.}
\begin{align*}
\psi_7 = & AG(q_{row} \rightarrow EXA[\ (\neg q_{row}Uq_{\sharp})\wedge \neg F(o \wedge \bigwedge_{i=0}^{n-1} b_i \wedge \neg b \wedge EXq_{\sharp}) \rightarrow \\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ G(o \wedge \bigwedge_{i=0}^{n-1} \neg b_i \rightarrow \bigvee_{t \in L} p_t)\ ]) 
\end{align*}
\newline
\newline
Finally we obtain the formula $\varphi_I$ as a conjunction of the formulas encoding the properties T1-T8 and W1-W7. It should be noticed that a model for $\varphi_I$ can contain multiple possible moves for player E on each position. In this case it suffices to choose one of the suggested moves because every rootpath without copy nodes represents a win for E.

Since in the formulas the nesting depth of conjunctions and disjunctions over all $t \in T$ or $b_i$ for $0 \leq i \leq n-1$ is constant, the length of $\varphi_I$ remains polynomial in $|I|$.   
%Finally we obtain the formula $\varphi_I = \bigwedge_{i=1}^{12} \chi_i \wedge \bigwedge_{i=1}^{6} \psi_i$.
%Since the nesting depth of conjunctions and disjunctions over all $t \in T$ or $b_i$ for $0 \leq i \leq n-1$ is constant, the length of $\varphi_I$ remains polynomial in $|I|$.
\newline
---------end-old-version-------------
\newline

==> compl-hctl+-temp.tex <==
\section{Satisfiability of \Honeplus} \label{sec:complexity}
\begin{theorem}\label{compl-lower-bound}
  Satisfiability of {\Honeplus} is hard for {\Texptime}. 
\end{theorem}

\begin{proof}
The proof is by reduction from a tiling game (with \Texptime complexity) to the satisfiability problem of
\Honeplus. Actually we show that the lower bound even holds for the fragment of \Honeplus without the
$\U$-operator.

An instance $I=(T,H,V,F,L,n)$ of the \emph{2EXP-corridor tiling game} consists of a finite set $T$ of \emph{tile
types}, two relations $H,V \subseteq T \times T$ which constitute the \emph{horizontal and vertical
constraints}, respectively, two sets $F,L \subseteq T$ which describe
the start and end conditions, respectively, and a number $n$
given in unary.

\thomas{Dass $n$ unär kodiert wird und wir dann
  $2^{2^n}$ verwenden, ist seltsam. Wir könnten $n$ binär kodieren und
bräuchten dann nur über $2^n$ zu reden. Am Ergebnis würde das nichts ändern.}
 The game is played by two players, $E$ and $A$, on a board consisting of $2^{(2^n)}$ columns
and (potentially) infinitely many rows. Starting with player $E$ and following the constraints $H$, $V$ and $F$ the
players put tiles to the board consecutively from left to right and row by row. The constraints prescribe the following conditions:
\begin{itemize}
\item A tile $t'$ can only be placed immediately to the right of a tile $t$ if $(t,t') \in H$.
\item A tile $t'$ can only be placed immediately above a tile $t$ if $(t,t') \in V$.
\item The types of all tiles in the first row belong to the set $F$. 
\end{itemize}
Player $E$ wins the game if a row is completed containing only tiles
from $L$ or if $A$ makes a move that violates the constraints. On the
other hand, player $A$ wins if $E$ makes a forbidden move or the game goes on ad infinitum.

A winning strategy for $E$ has to yield a countermove for all possible moves
of $A$ in all possible reachable situations. Furthermore, the starting condition and the horizontal and vertical constraints have to be respected.
Finally, the winning strategy must guarantee that either 
player $A$ comes into a situation where he can no longer make an
allowed move or a row with tiles from $L$ is completed.

The problem to decide for an instance $I$ whether player $E$ has a winning strategy on $I$ is complete for 
\Texptime \cite{Chlebus86}.\mthomas{In Chlebus steht das nicht
  explizit. Hier sollten wir genauer sein.}

We show in the following how to build a formula $\varphi_{I}$ of
polynomial length from an instance $|I|$ of the 2EXP-corridor tiling
game such that $\varphi_{I}$ is satisfiable if and only if player $E$
has a winning strategy in the game for $I$. In fact, a tree will
satisfy $\varphi_I$ if and only if it encodes a winning strategy of
player $E$.


\paragraph*{Encoding of the winning strategy for player $E$.} 
\mthomas{Der Zwischenraum wird kleiner, wenn sich die Seitengrenzen
  verschieben. Anpassungen per Hand sollten wir erst ganz am Ende vornehmen.}
We encode  strategies for player $E$ as  $T$-labeled trees in which each move is
represented by a sequence of nodes. The first move of player $E$ is represented by a sequence
starting at the root. Each sequence corresponding to a move of $E$ is followed by several branches, one
for every possible next move of $A$. Each sequence
corresponding to a move of $A$ is followed by one sequence of nodes
corresponding to the move of player $E$ following the strategy. It is clear that
such a tree represents a \emph{winning} strategy if every root path
corresponds to a sequence of moves resulting in a win for player
$E$.

In the encoding we use the propositions $\{\mathit{pos}_e, \mathit{pos}_u,b_0,...b_{n-1},\mathit{row}_e, \mathit{row}_u,b,$
$o,c,q_{\sharp}\} \cup \{p_t \ |\ t \in T\}$.  In order to be able to describe the constraints via a
\Honeplus-formula of polynomial length we serially number all positions of a row of the board in the
style of \cite{VardiS85}. While in \cite{VardiS85} a
row\footnote{Actually, the proof in \cite{VardiS85} uses alternating
  Turing machines and thus encodes configurations rather than rows.} consists of $2^n$ positions we have to
deal with $2^{2^n}$ positions in the current proof. We encode each
position by a sequence of $2^n$ nodes, each of which we call \emph{position
bits}. For each of these nodes the
propositions $b_0,...,b_{n-1}$ encode a binary number. Each position
bit in turn represents one bit of a binary
number of length $2^n$ via proposition $b$. Altogether, the
positions of a row are represented by a sequence of $2^n2^{2^n}$
nodes. We call a sequence of length $2^n$ representing one position of
the tiling a \emph{position sequence} and a sequence representing a
row a \emph{row sequence}.

For all nodes of a position sequence for a position carrying a tile of type $t$, the
proposition $p_t$ is true. For technical reasons, all position bits of
even positions are marked using the proposition $\mathit{pos}_e$,
those of odd positions
are marked with $\mathit{pos}_u$. Likewise, nodes in row sequences of
even rows are marked using $\mathit{row}_e$ while those of odd rows are
marked using $\mathit{row}_u$. 
%As in the proof of the \Dexptime-hardness of the satisfiability
%problem of \Hone \cite{Weber07} we serially number all positions of a
%row of the board in order to be able to describe the constraints via a
%\Honeplus-formula with polynomial leng
%
%To be able to distinguish between $2^{2^n}$ different positions with polynomial many propositions we encode each position via a sequence of $2^n$ nodes, called position bits. We construct an inner counter which serially numbers these position bits in binary via the propositions $b_0,...,b_{n-1}$. An outer counter treates then each of this position bits again as a bit of a binary number of lenght $2^n$. The proposition $b$ in a position bit decides whether the repective bit is set or not. After all we manage to count $2^{2^n}$ positions with $n+1$ propositions. 
%For each tile type $t\in T$ we use a proposition $p_t$. 
%For each even position there is an outgoing path for each possble move player $A$ can make. 
\thomas{Das Folgende verstehe ich nicht und habe es deshalb rausgenommen:
The nodes of
the part of the tree which do not belong to the encoding of the
winning strategy are labeled with $q_{\sharp}$.}

To be able to compare two nodes of large distance we use a technique that was originally invented in \cite{VardiS85} and was also applied 
%in the proof of the \Dexptime-hardness of the satisfiabilty problem of \CTLplus 
in \cite{JohannsenL03}. To this end, we use two kinds of nodes: \emph{original nodes} which are
labelled with the proposition $o$ and \emph{copy nodes} labelled with the proposition $c$.  For the
encoding of the winning strategy only the original nodes are relevant. Each original node has a copy
node with identical propositions (except for the proposition $o$) as a child. Likewise, each copy node
has only copy nodes with identical propositions as children (see Figure~\ref{winStrategy}). Copy nodes
will enable us to ''mark'' an original node $v$ by fixing a path $\pi$ through $v$ and its copy node
child. Since copy nodes carry the propositions of their parent
original nodes, assertions about an original node can be tested in any
of their subsequent copy nodes.

\paragraph{Testing vertical constraints.} 
The most difficult condition to test is that a tree respects the
vertical constraints. Thus, we have to check the following condition:
\emph{
  For every row,
  except the first one, the tile of every position is consistent with the
  tile of the same position in the previous row.}

To this end, we have to compare two position sequences representing corresponding positions in consecutive rows. To test that two 
sequences represent corresponding positions one has to check that
whenever two position bits are equivalent with respect to
$b_0,\ldots,b_{n-1}$, they are also equivalent with respect to
$b$. The technical challenge is to do this comparison with a formula
of linear (as opposed to exponential) size.
Finally, it has to be checked that the $p_t$ propositions of the two
position sequences are consistent. We give an informal description of the formula first.

Let $r'$ and $r$ be row sequences representing two consecutive rows.
Let $s$ be some position
sequence of $r$ for which consistence with the previous row
shall be checked. 

First we put the variable $x$ onto the last node of $s$. To ensure that a
position sequence $s'$ of $r'$ corresponds to $s$ we require for each
node $v'$ in $s'$ that there is a path starting in $v'$ which
eventually reaches the copy nodes of some node $v$ on $s$ such that $v'$
and (the copy nodes of) $v$ agree in $b_1,\ldots,b_n,b$. 
% Since on such a path the
% node $v$ can be considered as ''fixed'' and because the description of a path through a Boolean
% combination of temporal operators is allowed in \Honeplus the comparison of $v$ and $v'$ can be
% performed in the scope of a path quantifier without an exponential blowup in the formula length.

It is not hard to construct subformulas $\varphi_{\mathit{first}}$, $\psi_{\mathit{cur}}$ and 
$\mathit{step}_{\mathit{row}}$ describing the following.
\begin{itemize}
\item $\varphi_{\mathit{first}}$: The current node is the first bit of a position.
\item $\psi_{\mathit{cur}}$: The current path starts at a position bit, continues until the last bit of 
the position and follows then the copy nodes of the last bit. 
\item $\mathit{step}_{\mathit{row}}$: The current path contains exactly one of the propositions 
$\mathit{row}_e$ and $\mathit{row}_u$. Hence, it connects a row with the next one but not the one after
the next one etc. 
\end{itemize}
\ahmet{Wir sollten hier noch sagen, dass die Kodierung einer Position entlang eines \emph{eindeutigen} o-pfades durchgef\"uhrt wir.}
Then the vertical constraints can be formulated as follows:   
\begin{align*}
&\A\G[\varphi_{\mathit{first}} \rightarrow \bigwedge_{t' \in T}[p_{t'} \rightarrow \E[\psi_{\mathit{cur}} \wedge \F(o \wedge \bigwedge_{i=0}^{n-1}b_i \wedge \dx.@_{\myroot}\A\G[\xi \rightarrow \bigvee_{(t,t')\in V} p_t])]]] \\
&\xi = \varphi_f \wedge \E[\F x \wedge \G(\neg c \rightarrow \E\F x) \wedge \mathit{step}_{\mathit{row}}]\wedge \\
& \ \ \ \ \ \E[\psi_{\mathit{cur}}\wedge \G(o \rightarrow \E[\G(\neg c \rightarrow \F x)\wedge \F\E[\G\neg (\mathit{pos}_e \vee \mathit{pos}_u) \wedge \F x] \wedge \\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \bigwedge_{i=0}^{n-1} (b_i \leftrightarrow \F(c \wedge b_i)) \wedge b \leftrightarrow \F(c \wedge b)]) ]
\end{align*} 
%To exhaust the facilities of \CTLplus in order to be able to repeatedly refer to the propositions of a certain node on a path without using the variable $x$ we benefit from a coding technique which is also used in the proof of the \Dexptime-hardness of the satisfiability of \CTL \cite{JohannsenL03}. We add to each position bit the proposition $o$ (original) and append to it a subtree whose nodes are labelled exactly with the same propositions as the original position bit except that it is labelled with $c$ (copy) instead of $o$. Assumed there is a path fixed with the quantifier $E$ on which after some node only appear copy nodes then every copy represents the last original node on this path.       
\begin{figure}[t]
\begin{center}
\begin{pspicture}(-.2,-.1)(3,1) 
\wnode{1.5,.5}{A}
\wnode{2.5,.5}{B}
\wnode{3.5,.5}{C} 
\nccircle{<-}{A}{.2}
\ncline{B}{C}
\end{pspicture}
\end{center}
\label{winStrategy}
\caption{A path in the encoding of a winning strategy for player $E$}
\end{figure}
\qed
\end{proof}
----------begin-appendix-----------------------
\newline
%\input{compl-hctl+-old-version}
\newcommand{\ourcondition}[2]{#1: \emph{#2}}
Proof of Theorem \ref{compl-lower-bound}:
\begin{proof} 
We present the whole formula $\varphi_I$. It is composed of the conjunction of $\chi$ and $\psi$ where 
the first formula describes the basic tree structure that is needed to formulate a strategy and 
the second one guarantees that the model of $\varphi_I$ corresponds to a winning strategy for player $E$.
We first introduce some abbreviations: 
\begin{align*}
pos = &\mathit{pos}_e \vee \mathit{pos}_u &\\
row = &\mathit{row}_e \vee \mathit{row}_u &\\
\varphi_{\mathit{first}} =& o \wedge \bigwedge_{i=0}^{n-1} \neg b_i &\\
\psi_{\mathit{cur}} = &\G \neg p \wedge \F(c \wedge \bigwedge_{i=0}^{n-1} b_i)&\\
step_{pos} = &\F \mathit{pos}_e \wedge \neg \F \mathit{pos}_u \vee \F \mathit{pos}_u \wedge \neg \F \mathit{pos}_e &\\
\mathit{step}_{\mathit{row}} = &\F \mathit{row}_e \wedge \neg \F \mathit{row}_u \vee \F \mathit{row}_u \wedge \neg \F \mathit{row}_e&
\end{align*}
The first formula helps to describe some properties in a facile way.
\newline
\ourcondition{T1}{Each node of the tree is labelled with exactly one of the propositions $\mathit{row}_e$, $\mathit{row}_u$, $\mathit{pos}_e$, $\mathit{pos}_u$, $q_{\sharp}$, $o$ and $c$.} 
\begin{align*}
\chi_1 = \A\G [&(row \vee  pos \vee q_{\sharp} \vee o \vee c) \wedge \\ 
&(\mathit{pos}_e \rightarrow \neg \mathit{pos}_u \wedge \neg \mathit{row}_e \wedge \neg \mathit{row}_u \wedge \neg q_{\sharp} \wedge \neg o \wedge \neg c) \wedge  \\
&(\mathit{pos}_u \rightarrow \neg \mathit{pos}_e \wedge \neg \mathit{row}_e \wedge \neg \mathit{row}_u \wedge \neg q_{\sharp} \wedge \neg o \wedge \neg c) \wedge  \\
&(\mathit{row}_e \rightarrow \neg \mathit{pos}_e \wedge \neg \mathit{pos}_u \wedge \neg \mathit{row}_u \wedge \neg q_{\sharp} \wedge \neg o \wedge \neg c) \wedge  \\
&(\mathit{row}_u \rightarrow \neg \mathit{pos}_e \wedge \neg \mathit{pos}_u \wedge \neg \mathit{row}_e \wedge \neg q_{\sharp} \wedge \neg o \wedge \neg c) \wedge  \\
&(q_{\sharp} \rightarrow \neg \mathit{pos}_e \wedge \neg \mathit{pos}_u \wedge \neg \mathit{row}_e \wedge \neg \mathit{row}_u \wedge \neg o \wedge \neg c) \wedge \\
&(o \rightarrow \neg \mathit{pos}_e \wedge \neg \mathit{pos}_u \wedge \neg \mathit{row}_e \wedge \neg \mathit{row}_u \wedge \neg q_{\sharp} \wedge \neg c) \wedge \\         
&(c \rightarrow \neg \mathit{pos}_e \wedge \neg \mathit{pos}_u \wedge \neg \mathit{row}_e \wedge \neg \mathit{row}_u \wedge  \neg q_{\sharp} \wedge \neg o)]  
\end{align*}
\ourcondition{T2}{The root induces with the proposition $\mathit{row}_e$ the encoding of the first row and every node labelled with $\mathit{row}_e$ or $\mathit{row}_u$ has exactly one child labled with $\mathit{pos}_e$ signalising the encoding of a new position.}
\begin{align*} 
\chi_2 = \mathit{row}_e \wedge \A\G[row \rightarrow \E\X (\mathit{pos}_e \wedge \dx.@_{\myroot} \E\F(\E\X x \wedge \A\X x))]
\end{align*}
\ourcondition{T3}{Every child of a $\mathit{pos}_e$-or $\mathit{pos}_u$-node is labelled with the initial digit number.}
\begin{align*}
\chi_3 = \A\G[p \rightarrow \A\X\varphi_{\mathit{first}}]
\end{align*}
\ourcondition{T4}{As long as the last bit node of a position is not reached, the next node is labelled with the next digit number.}
\begin{align*} 
\chi_4 = \A\G&[o \wedge \neg \bigwedge _{i=0}^{n-1} b_i \rightarrow \\
&             \dx.\E\X(o \wedge \bigvee_{i=0}^{n-1} 
(\bigwedge _{j<i} (\neg b_j \wedge @_x b_j)\wedge b_i \wedge @_x \neg b_i \wedge \bigwedge _{j>i} (b_j \leftrightarrow @_x b_j)))]
\end{align*}
\ourcondition{T5}{Each position bit has a child, which represents a copy of it. The nodes of a subtree rooted at a copy node are labelled exactly with the same propositions.}
\begin{align*} 
\chi_5 = \A\G[&(o \rightarrow \dx. \E\X (c \wedge \bigwedge_{i=0}^{n-1}(b_i \leftrightarrow @_x b_i) \wedge b \leftrightarrow @_x b)) \wedge \\
&(c \rightarrow \dx.\A\G (c \wedge \bigwedge_{i=0}^{n-1}(b_i \leftrightarrow @_x b_i) \wedge b \leftrightarrow @_x b))]
\end{align*}
\ourcondition{T6}{Each position bit has exactly two children. One of them is its copy node and the other one is:  
\begin{itemize}
\item the next position bit if the current node is not already the last position bit or
\item a node containing one of the propositions $\mathit{pos}_e$, $\mathit{pos}_u$, $\mathit{row}_e$, $\mathit{row}_u$ and $q_{\sharp}$, otherwise.
\end{itemize}}
\begin{align*} 
\chi_{6a} = \A\G[o \wedge \neg \bigwedge_{i=0}^{n-1} b_i \rightarrow  &\E\X(o \wedge \dx. @_{root} \E\F(\E\X x \wedge \A\X(o \rightarrow x))) \wedge \\
                                                                 	    &\E\X(c \wedge \dx. @_{\myroot} \E\F(\E\X x \wedge \A\X(c \rightarrow x))) \wedge  \\
																																	    &\A\X(o \vee c)]
\end{align*}
\begin{align*}
\chi_{6b} = \A\G[o \wedge \bigwedge_{i=0}^{n-1} b_i \rightarrow &\E\X(c \wedge \dx. @_{\myroot}\E\F(\E\X x \wedge \A\X(c     			
                                                                \rightarrow x))) \wedge \\
																															 &\E\X(\neg c \wedge \dx. @_{\myroot}\E\F(\E\X x \wedge \A\X(\neg c     																																\rightarrow x))) \wedge \\
																															 &\A\X(c \vee pos \vee row \vee q_{\sharp})
\end{align*}
\ourcondition{T7}{With the propositions $\mathit{row}_e$ and $\mathit{row}_u$ the counting of the positions of the current row starts. This means that the next position gets the initial position number. Therefore the proposition $b$ is set to false in every bit node of this position.}
\begin{align*}
\chi_7 = \A\G[row \rightarrow \E\X\A\X\E[\psi_{\mathit{cur}} \wedge \G \neg b]]
\end{align*}
\newline
Compared to the increasing of a digit number the increasing of a position number is a little bit complicated because in the latter case the bits are distributed over several nodes. In addition, we have to account for the case that player $A$ cannot make a move without violating the horizontal or vertical constraints. In this case the game is over and $q_{\sharp}$-nodes follow only. We describe the increasing of a position number in three parts.
\newline
\ourcondition{T8a}{If the last position is reached then a new row is started or the game is over.}
\begin{align*}
\chi_{8a} &= \A\G[\varphi_{\mathit{first}} \wedge \E[\psi_{\mathit{cur}} \wedge \G b] \rightarrow \E[\G \neg p \wedge \F(o \wedge \bigwedge_{i = 0}^{n-1} b_i \wedge \E\X(row \vee q_{\sharp}))]]		
\end{align*}
\ourcondition{T8b}{If the last position is not reached and it is the turn of player $E$ then the next position definitely has to be encoded and it gets the next position number.}
\begin{align*}
\chi_{8b} =& \A\G[\varphi_{\mathit{first}} \wedge \E[\G \neg p \wedge \F(c \wedge \bigwedge_{i = 0}^{n-1} b_i \wedge b) ] \wedge \E[\psi_{\mathit{cur}} \wedge \F \neg b ] \rightarrow \theta]
\end{align*}
\textit{Find the bit which has to be switched.} 
\begin{align*}
\theta =& \E[\psi_{\mathit{cur}} \wedge \F(o \wedge \neg b \wedge \E\X(\neg c \wedge (o \rightarrow \E[\psi_{\mathit{cur}} \wedge \G b])) \wedge \theta')]
\end{align*}
\textit{Switch the same bit in the encoding of the next position.}
\begin{align*}
\theta' =& \dx.[\theta'' \wedge \E[\psi_{\mathit{cur}} \wedge \F(o \wedge \bigwedge_{i=0}^{n-1} b_i \wedge \\ 
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \E\X( pos \wedge \A\X\E[\psi_{\mathit{cur}} \wedge \F(o \wedge \bigwedge_{i=0}^{n-1} (b_i \leftrightarrow @_x b_i) \wedge (b \leftrightarrow @_x b) \wedge \\ 
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \E\X(\neg c \wedge (o \rightarrow \E[\psi_{\mathit{cur}} \wedge \G \neg b])))]))]] 
\end{align*}
\textit{Carry the values of the bits preceding the switched bit over to the encoding of the next position.}
\begin{align*}
\theta'' = & @_{\myroot}\E\F[\varphi_{\mathit{first}} \wedge \E[\G\neg p \wedge \F x \wedge \F(c \wedge \bigwedge_{i=0}^{n-1} (b_i \leftrightarrow @_x b_i)) \wedge \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \G(o \wedge \neg x \rightarrow \A[step_{pos} \wedge \bigwedge_{i=0}^{n-1} (b_i \leftrightarrow \F(c \wedge b_i)) \rightarrow b \leftrightarrow \F(c \wedge b)])]]
\end{align*}
\ourcondition{T8c}{If the last position is not reached and it is the turn of player $A$ then the next position has not necessarily to be encoded but the game could be over.}
\begin{align*}
\chi_{8c} = & \A\G[\varphi_{\mathit{first}} \wedge \E[\G \neg p \wedge \F(c \wedge \bigwedge_{i=0}^{n-1} b_i \wedge \neg b)] \rightarrow (\E[\psi_{\mathit{cur}} \wedge \F(o \wedge \bigwedge_{i=0}^{n-1}b_i \wedge \E\X q_{\sharp})]\vee \theta)]
\end{align*}
\ourcondition{T9}{Determining whether a position/row has an even or uneven number.}
\begin{align*}
\chi_{9a} = & \A\G[pos \rightarrow \dx.@_{\myroot}\A\G[pos \wedge \E\X\E[\psi_{\mathit{cur}} \wedge \F(o \wedge \bigwedge_{i=0}^{n-1} b_i \wedge \E\X x)] \rightarrow \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ (\mathit{pos}_e \leftrightarrow @_x \mathit{pos}_u)]] \\ \\
\chi_{9b} = & \A\G[row \rightarrow \dx.@_{\myroot}\A\G[row \wedge \E\X\E[\G\neg row \wedge \F(c \wedge \bigwedge_{i=0}^{n-1} b_i) \wedge \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \F(o \wedge \bigwedge_{i=0}^{n-1} b_i \wedge \E\X x)] \rightarrow (\mathit{row}_e \leftrightarrow @_x \mathit{row}_u)]] \\
\end{align*}

Now we use the tree structure described above to encode a winning strategy for player $E$.
\newline
\ourcondition{W1}{The game ends after a finite sequence of moves.}
\newline
We express this by postulating that on every rootpath which does not contain any copy nodes a $q_{\sharp}$-node is eventually reached. A $q_{\sharp}$-node is followed only by $q_{\sharp}$-nodes.
\begin{align*}
\psi_1 = & \A(\G \neg c \rightarrow \F q_{\sharp}) \wedge \A\G(q_{\sharp} \rightarrow \A\G q_{\sharp}) 
\end{align*}
\ourcondition{W2}{To each position belongs exactly one tile type.}
\newline
We remember that a tile type $t$ is represented by the proposition $p_t$ in the first bit node of the corresponding position.
\begin{align*}
\psi_2 = & \A\G[\varphi_{\mathit{first}} \rightarrow \bigvee_{t \in T}(p_t \wedge \bigwedge_{t \neq t'\in T}\neg p_{t'} )]
\end{align*}
\ourcondition{W3}{According to the horizontal constraints, the tile type of every position, except the first one on each row, is convenient to the tile type of the precedent position.}
\begin{align*}
\psi_3 = & \A\G[\varphi_{\mathit{first}}  \rightarrow \\
&\ \ \ \ \ \bigwedge_{t' \in T}[p_{t'} \rightarrow \dx.@_{\myroot}\A\G[\varphi_{\mathit{first}} \wedge \neg x\wedge \E[\F x \wedge step_p \wedge \G\neg row]\rightarrow \bigvee_{(t,t')\in H} p_t]]]
\end{align*}
\ourcondition{W4}{According to the vertical constraints, for every row, except the first one, it holds that the tile type of every position on this row is convenient to the tile type of the same position on the precedent row.}
\begin{align*}
\psi_4 =&\A\G[\varphi_{\mathit{first}} \rightarrow \bigwedge_{t' \in T}[p_{t'} \rightarrow \E[\psi_{\mathit{cur}} \wedge \F(o \wedge \bigwedge_{i=0}^{n-1}b_i \wedge \dx.@_{\myroot}\A\G[\xi \rightarrow \bigvee_{(t,t')\in V} p_t])]]] \\
\xi = &\varphi_{\mathit{first}} \wedge \E[\F x \wedge \G(\neg c \rightarrow \E\F x) \wedge \mathit{step}_{\mathit{row}}]\wedge \\
&\E[\psi_{\mathit{cur}}\wedge \G(o \rightarrow \E[\G(\neg c \rightarrow \F x)\wedge \F\E[\G\neg pos \wedge \F x] \wedge \\
& \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \bigwedge_{i=0}^{n-1} (b_i \leftrightarrow \F(c \wedge b_i)) \wedge b \leftrightarrow \F(c \wedge b)]) ]
\end{align*}
\ourcondition{W5}{All possible moves of player $A$ are represented in the encoding.}
\begin{align*}
\psi_5 =& \A\G[\varphi_{\mathit{first}} \wedge \E[\psi_{\mathit{cur}} \wedge \F(o \wedge \bigwedge_{i=0}^{n-1}b_i \wedge \neg b)] \rightarrow \\
&\ \ \ \ \ \ \bigwedge_{t \in T}(p_t \rightarrow \bigwedge_{(t,t')\in H}(\E[\psi_{\mathit{cur}} \wedge \F(o \wedge \bigwedge_{i=0}^{n-1} b_i \wedge \E\X(pos \wedge \E\X p_{t'}))] \vee \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \E[\psi_{\mathit{cur}} \wedge \F(o \wedge \bigwedge_{i=0}^{n-1}b_i \wedge \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \dx.@_{\myroot}\E\F(\xi \wedge \\ 
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \bigvee_{(t'',t')\notin V}\E[\psi_{\mathit{cur}} \wedge \\
&\ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \ \F(o \wedge \bigwedge_{i=0}^{n-1}b_i \wedge \E\X (p_{t''} \wedge \E\F x))]))]))] 
\end{align*}
\ourcondition{W6}{All tile types in the first row are from the set $F$.}
\begin{align*}
\psi_6 = \A\G[\varphi_{\mathit{first}} \wedge \dx.@_{\myroot}\E\X\E[\G\neg row \wedge \F x] \rightarrow \bigvee_{t \in F} p_t]
\end{align*}
\ourcondition{W7}{Unless the game terminates prematurely (because player $A$ is not able to make a further move) all tile types in the last row are from the set $L$.}
\begin{align*}
\psi_7 = & \A\G[o \wedge \bigwedge_{i=0}^{n-1} b_i \wedge b \wedge \E\X q_{\sharp} \rightarrow \\
&\ \ \ \ \ \dx.@_{\myroot}\E\F[row \wedge \E\X\E[\G \neg row \wedge \F x \wedge \G(\varphi_{\mathit{first}} \rightarrow \bigvee_{t \in L} p_t)]]]
\end{align*}
\newline
\newline
Finally we obtain the formula $\varphi_I$ as a conjunction of the formulas encoding the properties T1-T9 and W1-W7. It should be noticed that a model for $\varphi_I$ can contain multiple possible moves for player $E$ on each position. In this case it suffices to choose one of the suggested moves because every rootpath without copy nodes represents a win for $E$.

Since in the formulas the nesting depth of conjunctions and disjunctions over all $t \in T$ or $b_i$ for $0 \leq i \leq n-1$ is constant, the length of $\varphi_I$ remains polynomial in $|I|$.
\qed
\end{proof}
----------end-appendix-----------------------

We can obtain, by simple instantiation, a consequence of this lower complexity bound which will
be useful later on in proving the exponential succinctness gap between \Honeplus and \Hone.

\begin{corollary}
\label{cor:deepmodels}
There are finitely satisfiable \Honeplus formulas $\varphi_n$, $n \in \Nat$, of size $\bigO(n)$ s.t.\ 
every tree model $\mathcal{T}_n$ of $\varphi_n$ has height at least $2^{2^{2^n}}$.
\end{corollary}

\begin{proof}
(Sketch) It is not difficult to construct instances $I_n$, $n \in \Nat$, of the 2EXP-tiling game for which
player $E$ has a winning strategy such that any successful tiling of the $2^{2^n}$-corridor requires 
$2^{2^{2^n}}$ rows. In order to achieve this, one encodes bits using tiles and forms the constraints in a
way that enforces the first row to encode the number $0$ in binary of length $2^{2^n}$, and each other row to
encode the successor in the natural number of the preceding row, while winning requires the number 
$2^{2^{2^n}}$ to be reached. 

The construction in the proof of Thm.~\ref{compl-lower-bound} maps each $I_n$ to a formula $\varphi_n$ of
size $\bigO(n)$ that is finitely satisfiable such that every finite model $\mathcal{T}_n$ of $\varphi_n$ 
encodes a winning strategy for player $E$ in the $2^{2^n}$-tiling game. Such a strategy will yield a 
successful tiling of the $2^{2^n}$-corridor for any counterstrategy of player $A$, and any such tiling is 
encoded on a path of $\mathcal{T}_n$ which contains each row of length $2^{2^n}$ as a segment of which 
there are $2^{2^{2^n}}$ many. Thus, $\mathcal{T}_n$ has to have height at least $2^{2^n}\cdot 2^{2^{2^n}}$.
\qed
\end{proof}

----------begin-appendix-----------------------
\newline
\newcommand{\blow}{{\mathtt{l}}}
\newcommand{\bflip}{{\mathtt{f}}}
\newcommand{\bstay}{{\mathtt{s}}}
Proof of Corollary~\ref{cor:deepmodels}:
\begin{proof} 
Consider the following instances of the 2EXP-tiling game: $I_n := (T,H,V,F,L,n)$ where $T = \{0,1\}
\times \{\blow,\bflip,\bstay\}$. Tiles are supposed to model bit values in their first component. The second
component describes whether or not a bit has to be \emph{flipped} (value $\bflip$) or remains the
\emph{same} (value $\bstay$) in the increase of a value encoded in binary through these bits. The value
$\blow$ is used to mark the \emph{lowest} bit in a number. Remember that in binary increase the lowest
bit always gets flipped whereas the flipping of any other bit is determined by the value of itself,
the value of the next lower bit and the question whether or not that bit gets flipped. We denote a
tile as $0^\blow$ for instance rather than $(0,\blow)$.

$I_n$ is constructed in a way that forces both players to put down the number $0$ in binary coding
into the first row of the $2^{2^n}$-arena and, whenever a row encodes a number $i$, then the players
need to place the binary encoding of $i+1$ into the next row. Thus, there will be (almost) no choices
for the players. Player $E$ should win when the highest possible number $2^{2^{2^n}}$ is placed in a
row. 

The starting constraints are $F := \{ 0^\blow, 0^\bstay \}$. Hence, the first row
must encode $0$. The horizontal constraints are as follows.
\begin{displaymath}
H \enspace := \enspace \{ (0^\blow,b^\bstay), (1^\blow,b^\bflip), (0^\bflip,b^\bstay), (1^\bflip,b^\bflip), 
(0^\bstay,b^\bstay), (1^\bstay,b^\bstay) \}
\end{displaymath}
where $b$ is, in any case, an arbitrary value in $\{0,1\}$.

Now note that with this $H$ and $F$, there are only two possible first rows that the players can lay down:
$0^\blow 0^\bstay \ldots 0^\bstay$ or $0^\bstay \ldots 0^\bstay$, and it is player $E$ who determines 
entirely through his first choice which of these it is going to be.

Next we will translate the informal description of binary increase given above into the vertical
constraints.
\begin{displaymath}
V \enspace := \enspace \{ (0^\blow,1^\blow), (1^\blow,0^\blow), (0^\bflip,1^x), (1^\bflip,0^x), (0^\bstay,0^x), 
(1^\bstay,1^x) \}
\end{displaymath}
where $x$ is, in any case this time, an arbitrary value in $\{\bflip,\bstay\}$.

Now note that, if a row $i$ is layed down entirely, then the vertical constraints determine uniquely the
bit value of each tile in the next row. Furthermore, if the first tile in row $i$ is of the form 
$b^\blow$ then the first tile in row $i+1$ is uniquely determined to be $(1-b)^\blow$, and $H$ as well
as the bit values in row $i+1$ uniquely determine the flip-values of all the bits in row $i+1$. Furthermore,
all lowest bits that are all $1$ in row $i$ are $0$ in row $i+1$, the lowest bit that is $0$ in row $i$ is
$1$ in row $i+1$, and all other bits in row $i+1$ retain their value from row $i$. Hence, if row $i$
encodes the number $i$ in binary (starting with $0$), then row $i+1$ encodes the number $i+1$ in binary.

Thus, if player $E$ chooses tile $0^\blow$ as the first one, then both players have no choice but to
lay down the binary encodings of $0,1,2,\ldots$. On the other hand, if player $E$ chooses tile $0^\bstay$
as the first one then all rows will encode the number $0$ because the entire arena must be tiled with
$0^\bstay$ only. 

Finally, remember that the goal is to construct $I_n$ in a way that enforces a play filling $2^{2^{2^n}}$ many
rows. This can now easily be achieved by constuction the end constraints in a way that player $E$ only
wins when the number $2^{2^{2^n}}-1$ has been placed down in a row. We therefore set $L := \{ 1^\blow, 1^\bflip \}$.
Note that in the successive increase as constructed above, the last row cannot contain the tile $1^\bstay$. \qed
\end{proof}



----------end-appendix-----------------------

%%% Local Variables: 
%%% mode: latex
%%% TeX-master: "start.tex"
%%% End: 

